Distinguishing Commercial from Editorial Content in News

How can we distinguish commercial from editorial content in news, or more specifically, differentiate between advertorials and regular news articles? An advertorial is a commercial message written and formatted as an article, making it harder for readers to recognize these as advertising, despite the use of disclaimers. In our research we aim to differentiate the two using a machine learning model, and a lexicon derived from it. This was accomplished by scraping 1.000 articles and 1.000 advertorials from four different Dutch news sources and classifying these based on textual features. With this setup our most successful machine learning model had an accuracy of just over $90\%$. To generate additional insights into differences between news and advertorial language, we also analyzed model coefficients and explored the corpus through co-occurrence networks and t-SNE graphs.

==> graphs/graph1.tex <==
\pgfdeclarelayer{nodelayer}
\pgfdeclarelayer{edgelayer}
\pgfsetlayers{edgelayer, nodelayer}
\begin{figure}[h]
\centering
\resizebox{12.5cm}{!}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [main node] (5) at (0, 0) {Trump};
		\node [main node] (7) at (6, -4) {coronavirus};
		\node [main node] (8) at (-6, 4) {politiek};
		\node [main node] (10) at (11, -4) {liveblog};
		\node [main node] (11) at (6, -9) {verspreidt};
		\node [main node] (12) at (9, -12) {hoestdruppeltjes};
		\node [main node] (13) at (-6, 9) {belang};
		\node [main node] (14) at (-11, 4) {politieke};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=150, out=-30] (5.center) to (7.center);
		\draw (5.center) to (8.center);
		\draw (11.center) to (7.center);
		\draw (10.center) to (7.center);
		\draw (14.center) to (8.center);
		\draw (8.center) to (13.center);
		\draw (11.center) to (12.center);
	\end{pgfonlayer}
\end{tikzpicture}
}
\break
\caption{Important connections from the main editorial cluster}
\end{figure}

==> graphs/graph2.tex <==
\pgfdeclarelayer{nodelayer}
\pgfdeclarelayer{edgelayer}
\pgfsetlayers{edgelayer, nodelayer}
\begin{figure}
\centering
\resizebox{12.5cm}{!}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [comm node] (0) at (2, 2) {nieuw};
		\node [comm node] (1) at (-2, -2) {nieuwe};
		\node [summ node] (2) at (4, -4) {nodes referring to products};
		\node [summ node] (3) at (-4, 4) {nodes referring to business operations};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (3.center) to (0.center);
		\draw (3.center) to (1.center);
		\draw (0.center) to (2.center);
		\draw (1.center) to (2.center);
	\end{pgfonlayer}
\end{tikzpicture}
}
\break
\caption{Important connections from the main commercial cluster}
\end{figure}

==> graphs/graph3.tex <==
\pgfdeclarelayer{nodelayer}
\pgfdeclarelayer{edgelayer}
\pgfsetlayers{edgelayer, nodelayer}
\begin{figure}
\centering
\resizebox{12.5cm}{!}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [comm node] (0) at (0, 0) {ontdek};
		\node [comm node] (1) at (0, 2) {disney};
		\node [comm node] (2) at (-2.25, 0) {mogelijkheden};
		\node [comm node] (3) at (-2.25, 3.25) {thailand};
		\node [comm node] (4) at (-4, 2) {toerisme};
		\node [comm node] (5) at (0, 5) {informatie};
		\node [comm node] (7) at (6, -2) {venlo};
		\node [comm node] (8) at (9, -2) {lichaam};
		\node [comm node] (9) at (8, -4) {ontdekte};
		\node [comm node] (10) at (4, -4) {leven};
		\node [comm node] (11) at (1, -3) {kerst};
		\node [comm node] (12) at (-5.5, -2.5) {bedrijfsoverdracht};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (7.center) to (8.center);
		\draw (7.center) to (9.center);
		\draw (10.center) to (7.center);
		\draw (11.center) to (7.center);
		\draw (7.center) to (0.center);
		\draw (0.center) to (1.center);
		\draw (2.center) to (1.center);
		\draw (2.center) to (3.center);
		\draw (4.center) to (3.center);
		\draw (3.center) to (5.center);
		\draw (1.center) to (5.center);
		\draw (2.center) to (12.center);
	\end{pgfonlayer}
\end{tikzpicture}
}
\break
\caption{Commercial cluster that centers around tourism}
\end{figure}

==> graphs/graph4.tex <==
\pgfdeclarelayer{nodelayer}
\pgfdeclarelayer{edgelayer}
\pgfsetlayers{edgelayer, nodelayer}
\begin{figure}
\centering
\resizebox{12.5cm}{!}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [main node] (0) at (0, 0) {milde};
		\node [main node] (1) at (-2, -3) {meeste};
		\node [main node] (2) at (5, -1) {griep};
		\node [main node] (3) at (2, 4) {klacht};
		\node [main node] (4) at (-5, 1) {griepachtige};
		\node [main node] (5) at (-3, 4) {klachten};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (1.center) to (0.center);
		\draw (0.center) to (3.center);
		\draw (0.center) to (2.center);
		\draw (0.center) to (4.center);
		\draw (4.center) to (5.center);
		\draw (5.center) to (2.center);
		\draw (4.center) to (3.center);
		\draw (4.center) to (1.center);
		\draw (1.center) to (2.center);
		\draw (2.center) to (3.center);
		\draw (0.center) to (5.center);
	\end{pgfonlayer}
\end{tikzpicture}
}
\break
\caption{Editorial cluster that centers around covid symptoms}
\end{figure}
